Deep Probabilistic Movement Primitives with a Bayesian Aggregator

Movement primitives are trainable parametric models that reproduce robotic movements starting from a limited set of demonstrations. Previous works proposed simple linear models that exhibited high sample efficiency and generalization power by allowing temporal modulation of movements (reproducing movements faster or slower), blending (merging two movements into one), via-point conditioning (constraining a movement to meet some particular via-points) and context conditioning (generation of movements based on an observed variable, e.g., position of an object). Previous works have proposed neural network-based motor primitive models, having demonstrated their capacity to perform tasks with some forms of input conditioning or time-modulation representations. However, there has not been a single unified deep motor primitive's model proposed that is capable of all previous operations, limiting neural motor primitive's potential applications. This paper proposes a deep movement primitive architecture that encodes all the operations above and uses a Bayesian context aggregator that allows a more sound context conditioning and blending. Our results demonstrate our approach can scale to reproduce complex motions on a larger variety of input choices compared to baselines while maintaining operations of linear movement primitives provide.

==> figures/close-drawer.tex <==
\begin{tikzpicture}
	\node (cartpole) at (0,0) {\includegraphics[height=4cm]{figures/close-drawer.png}};
	\node [above=0pt of cartpole.north] {\small{(a)}};
%	\node [below=.45cm of cartpole.south] {};
\end{tikzpicture}


==> figures/kinova_fig_1_try.tex <==
\begin{tikzpicture}
    \node (cartpole) at (0,0) {\includegraphics[width=6.2cm, trim=1cm 5cm 0cm 3cm,clip]{figures/kinova_pick_n_place.pdf}};
	%\node (cartpole) at (0,0) {\includegraphics[height=3.2cm, trim=0cm 3cm 3cm 0cm,clip]{figures/kinova_pick_n_place.pdf}};
	\node [above=0pt of cartpole.north] {\small{(c)}};
%	\node [below=.45cm of cartpole.south] {};
\end{tikzpicture}

==> figures/shaking.tex <==
\begin{tikzpicture}
	\node (cartpole) at (0,0) {\includegraphics[height=3.2cm, trim=3cm 3cm 3cm 0cm,clip]{figures/shaking_task.pdf}};
	\node [above=0pt of cartpole.north] {\small{(d)}};
%	\node [below=.45cm of cartpole.south] {};
\end{tikzpicture}


==> figures/trash-task-side.tex <==
\begin{tikzpicture}
	\node (cartpole) at (0,0) {\includegraphics[angle=90, height=3.2cm,trim=10cm 5cm 18cm 0cm,clip]{figures/plane_shot_of_pick_and_place.JPG}};
	\node [above=0pt of cartpole.north] {\small{(d)}};
	%	\node [below=.45cm of cartpole.south] {};
\end{tikzpicture}


==> figures/trash-task-top.tex <==
\begin{tikzpicture}
	\node (cartpole) at (0,0) {\includegraphics[height=3.2cm, trim=0cm 3cm 23cm 0cm,clip]{figures/trash-task-top.pdf}};
	\node [above=0pt of cartpole.north] {\small{(c)}};
%	\node [below=.45cm of cartpole.south] {};
\end{tikzpicture}


==> figures/via_pt_opt/opt_curv_keypt_cond_backup.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
title={\small  Accuracy of Via-Point Conditioning},
title style = {yshift=-5pt},
legend cell align={left},
legend columns=2,
height=5cm,
width=8.8cm,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204, at={(-0,-0.3)}, anchor=north west, font=\small},%, at=(axis cs:0.5,1)},
tick align=outside,
tick pos=left,
grid=both,
x grid style={darkgray176},
xlabel={\small Iterations},
xmin=-9.54773869346734, xmax=200.502512562814,
xtick style={color=black, draw=none},
y grid style={darkgray176},
ylabel={\small MSE (Log Scale)},
ylabel near ticks,
ylabel style={yshift=-10pt},
ymin=-8.73282400878992, ymax=1.73848536986873,
ytick style={color=black, draw=none},
xticklabel style={font=\scriptsize, yshift=5pt},
yticklabel style={font=\scriptsize, xshift=5pt}
]
\path [draw=blue, fill=blue, opacity=0.25]
(axis cs:0,1.26251676174788)
--(axis cs:0,1.22927931818541)
--(axis cs:10.0502512562814,1.16524207075094)
--(axis cs:20.1005025125628,1.09813360910662)
--(axis cs:30.1507537688442,1.02754069689505)
--(axis cs:40.2010050251256,0.953519643801313)
--(axis cs:50.251256281407,0.875815945520235)
--(axis cs:60.3015075376884,0.794682127753071)
--(axis cs:70.3517587939699,0.709683962436421)
--(axis cs:80.4020100502512,0.620870629767231)
--(axis cs:90.4522613065326,0.528650182442954)
--(axis cs:100.502512562814,0.432620851090192)
--(axis cs:110.552763819095,0.333345104919023)
--(axis cs:120.603015075377,0.230457203271856)
--(axis cs:130.653266331658,0.124124726167548)
--(axis cs:140.70351758794,0.0146835360516094)
--(axis cs:150.753768844221,-0.0978477552915011)
--(axis cs:160.804020100502,-0.213672491452641)
--(axis cs:170.854271356784,-0.332189525043487)
--(axis cs:180.904522613065,-0.453349125076386)
--(axis cs:190.954773869347,-0.577539092757881)
--(axis cs:190.954773869347,-0.515285117342144)
--(axis cs:190.954773869347,-0.515285117342144)
--(axis cs:180.904522613065,-0.393197006843908)
--(axis cs:170.854271356784,-0.273903430056122)
--(axis cs:160.804020100502,-0.157337431945997)
--(axis cs:150.753768844221,-0.0434577869898304)
--(axis cs:140.70351758794,0.0672677780148479)
--(axis cs:130.653266331658,0.174929638764456)
--(axis cs:120.603015075377,0.279540558304617)
--(axis cs:110.552763819095,0.380765233558493)
--(axis cs:100.502512562814,0.47839377047331)
--(axis cs:90.4522613065326,0.572847286653983)
--(axis cs:80.4020100502512,0.66363134163751)
--(axis cs:70.3517587939699,0.75101098746096)
--(axis cs:60.3015075376884,0.834620339656843)
--(axis cs:50.251256281407,0.91455040779287)
--(axis cs:40.2010050251256,0.991051076179688)
--(axis cs:30.1507537688442,1.06390867182542)
--(axis cs:20.1005025125628,1.13338806688677)
--(axis cs:10.0502512562814,1.19948508689935)
--(axis cs:0,1.26251676174788)
--cycle;

\path [draw=red, fill=red, opacity=0.25]
(axis cs:0,-3.80852540719057)
--(axis cs:0,-3.87109837613138)
--(axis cs:10.0502512562814,-4.00305217365785)
--(axis cs:20.1005025125628,-4.20239444572153)
--(axis cs:30.1507537688442,-4.39204524897719)
--(axis cs:40.2010050251256,-4.57138081967108)
--(axis cs:50.251256281407,-4.79847942860484)
--(axis cs:60.3015075376884,-4.91037267183033)
--(axis cs:70.3517587939699,-5.16894725817265)
--(axis cs:80.4020100502512,-5.19241835087237)
--(axis cs:90.4522613065326,-5.39229972685486)
--(axis cs:100.502512562814,-5.36339094367944)
--(axis cs:110.552763819095,-5.60030979778246)
--(axis cs:120.603015075377,-5.63510449840258)
--(axis cs:130.653266331658,-5.74684249149254)
--(axis cs:140.70351758794,-5.92171608004421)
--(axis cs:150.753768844221,-6.0681330158801)
--(axis cs:160.804020100502,-6.11469769364935)
--(axis cs:170.854271356784,-6.20760623800996)
--(axis cs:180.904522613065,-6.33380810851053)
--(axis cs:190.954773869347,-6.55580074414042)
--(axis cs:190.954773869347,-6.4008543594644)
--(axis cs:190.954773869347,-6.4008543594644)
--(axis cs:180.904522613065,-6.23401281981045)
--(axis cs:170.854271356784,-6.11159220193509)
--(axis cs:160.804020100502,-6.00438356606019)
--(axis cs:150.753768844221,-5.93569993425647)
--(axis cs:140.70351758794,-5.82525782321988)
--(axis cs:130.653266331658,-5.65256900490755)
--(axis cs:120.603015075377,-5.55093110118838)
--(axis cs:110.552763819095,-5.49466142242566)
--(axis cs:100.502512562814,-5.27976966090384)
--(axis cs:90.4522613065326,-5.29337084978563)
--(axis cs:80.4020100502512,-5.11078436984074)
--(axis cs:70.3517587939699,-5.07102845085217)
--(axis cs:60.3015075376884,-4.82363802277908)
--(axis cs:50.251256281407,-4.7208522083851)
--(axis cs:40.2010050251256,-4.50470281036109)
--(axis cs:30.1507537688442,-4.33025548673814)
--(axis cs:20.1005025125628,-4.14158187907396)
--(axis cs:10.0502512562814,-3.9454745043855)
--(axis cs:0,-3.80852540719057)
--cycle;

\path [draw=blue, fill=blue, opacity=0.25]
(axis cs:0,-1.3288210029745)
--(axis cs:0,-1.41661038683952)
--(axis cs:10.0502512562814,-1.67105616834687)
--(axis cs:20.1005025125628,-1.92655082838651)
--(axis cs:30.1507537688442,-2.19183867528162)
--(axis cs:40.2010050251256,-2.45774067254302)
--(axis cs:50.251256281407,-2.71899562849387)
--(axis cs:60.3015075376884,-2.98201925096039)
--(axis cs:70.3517587939699,-3.23688584063405)
--(axis cs:80.4020100502512,-3.49426676622936)
--(axis cs:90.4522613065326,-3.74594717538059)
--(axis cs:100.502512562814,-3.99078004366334)
--(axis cs:110.552763819095,-4.23276038203661)
--(axis cs:120.603015075377,-4.46808230468435)
--(axis cs:130.653266331658,-4.68925499737801)
--(axis cs:140.70351758794,-4.89300709316589)
--(axis cs:150.753768844221,-5.10572993264923)
--(axis cs:160.804020100502,-5.29736062913796)
--(axis cs:170.854271356784,-5.45491086000244)
--(axis cs:180.904522613065,-5.59389689322233)
--(axis cs:190.954773869347,-5.75296880603447)
--(axis cs:190.954773869347,-5.61276156002837)
--(axis cs:190.954773869347,-5.61276156002837)
--(axis cs:180.904522613065,-5.45949722969052)
--(axis cs:170.854271356784,-5.32145788045045)
--(axis cs:160.804020100502,-5.1670954633821)
--(axis cs:150.753768844221,-4.98068108715035)
--(axis cs:140.70351758794,-4.77468021419811)
--(axis cs:130.653266331658,-4.57144351667603)
--(axis cs:120.603015075377,-4.3490435042987)
--(axis cs:110.552763819095,-4.11371026867392)
--(axis cs:100.502512562814,-3.8690411656762)
--(axis cs:90.4522613065326,-3.62190573413889)
--(axis cs:80.4020100502512,-3.3702417474298)
--(axis cs:70.3517587939699,-3.11014699768403)
--(axis cs:60.3015075376884,-2.85702257806774)
--(axis cs:50.251256281407,-2.59662957703725)
--(axis cs:40.2010050251256,-2.33787887156303)
--(axis cs:30.1507537688442,-2.07893616447497)
--(axis cs:20.1005025125628,-1.82151001687783)
--(axis cs:10.0502512562814,-1.57362696145593)
--(axis cs:0,-1.3288210029745)
--cycle;

\path [draw=red, fill=red, opacity=0.25]
(axis cs:0,-5.72492937703481)
--(axis cs:0,-5.84243530658776)
--(axis cs:10.0502512562814,-6.3536143667341)
--(axis cs:20.1005025125628,-6.76216038869553)
--(axis cs:30.1507537688442,-7.07202345932222)
--(axis cs:40.2010050251256,-7.23965769504057)
--(axis cs:50.251256281407,-7.38400832865288)
--(axis cs:60.3015075376884,-7.54393899455192)
--(axis cs:70.3517587939699,-7.57390076546064)
--(axis cs:80.4020100502512,-7.68013921087273)
--(axis cs:90.4522613065326,-7.77373675122771)
--(axis cs:100.502512562814,-7.87989429350193)
--(axis cs:110.552763819095,-7.89018546677651)
--(axis cs:120.603015075377,-7.96770036728606)
--(axis cs:130.653266331658,-8.06733052422245)
--(axis cs:140.70351758794,-8.00271979940747)
--(axis cs:150.753768844221,-8.13279321256465)
--(axis cs:160.804020100502,-8.0944090315102)
--(axis cs:170.854271356784,-8.19403826958276)
--(axis cs:180.904522613065,-8.18306111256556)
--(axis cs:190.954773869347,-8.25685540066907)
--(axis cs:190.954773869347,-8.16021662648125)
--(axis cs:190.954773869347,-8.16021662648125)
--(axis cs:180.904522613065,-8.10122607412628)
--(axis cs:170.854271356784,-8.1154965035909)
--(axis cs:160.804020100502,-8.0035337045112)
--(axis cs:150.753768844221,-8.05952736813147)
--(axis cs:140.70351758794,-7.89704736927879)
--(axis cs:130.653266331658,-7.99476816512731)
--(axis cs:120.603015075377,-7.88758690288125)
--(axis cs:110.552763819095,-7.80982016397436)
--(axis cs:100.502512562814,-7.79125950298425)
--(axis cs:90.4522613065326,-7.6821893703404)
--(axis cs:80.4020100502512,-7.59673998523072)
--(axis cs:70.3517587939699,-7.47550467589034)
--(axis cs:60.3015075376884,-7.43586993491193)
--(axis cs:50.251256281407,-7.27089503792243)
--(axis cs:40.2010050251256,-7.11934056581185)
--(axis cs:30.1507537688442,-6.95690609757408)
--(axis cs:20.1005025125628,-6.64868737800897)
--(axis cs:10.0502512562814,-6.22101470444587)
--(axis cs:0,-5.72492937703481)
--cycle;

\path [draw=blue, fill=blue, opacity=0.25]
(axis cs:0,-0.277699396817483)
--(axis cs:0,-0.334980911975377)
--(axis cs:10.0502512562814,-0.520936972760644)
--(axis cs:20.1005025125628,-0.731945771992418)
--(axis cs:30.1507537688442,-0.944524277824716)
--(axis cs:40.2010050251256,-1.13374378804243)
--(axis cs:50.251256281407,-1.32302506473992)
--(axis cs:60.3015075376884,-1.48797664498802)
--(axis cs:70.3517587939699,-1.65001094306786)
--(axis cs:80.4020100502512,-1.79274379993625)
--(axis cs:90.4522613065326,-1.93549632833306)
--(axis cs:100.502512562814,-2.06432925580419)
--(axis cs:110.552763819095,-2.19815610143823)
--(axis cs:120.603015075377,-2.31926076088125)
--(axis cs:130.653266331658,-2.43613356562949)
--(axis cs:140.70351758794,-2.54722211480664)
--(axis cs:150.753768844221,-2.66170634616768)
--(axis cs:160.804020100502,-2.77479068007812)
--(axis cs:170.854271356784,-2.87165635475976)
--(axis cs:180.904522613065,-2.97405014811697)
--(axis cs:190.954773869347,-3.06923599058822)
--(axis cs:190.954773869347,-2.94316065908209)
--(axis cs:190.954773869347,-2.94316065908209)
--(axis cs:180.904522613065,-2.84940251357353)
--(axis cs:170.854271356784,-2.75035804992176)
--(axis cs:160.804020100502,-2.6546659838598)
--(axis cs:150.753768844221,-2.54499521737772)
--(axis cs:140.70351758794,-2.43396457828226)
--(axis cs:130.653266331658,-2.32377507279084)
--(axis cs:120.603015075377,-2.20822141674661)
--(axis cs:110.552763819095,-2.08829009507178)
--(axis cs:100.502512562814,-1.95745263350753)
--(axis cs:90.4522613065326,-1.82948127339262)
--(axis cs:80.4020100502512,-1.69011495342923)
--(axis cs:70.3517587939699,-1.5481320342406)
--(axis cs:60.3015075376884,-1.38926656093035)
--(axis cs:50.251256281407,-1.22579993104843)
--(axis cs:40.2010050251256,-1.04333615523714)
--(axis cs:30.1507537688442,-0.859034177460096)
--(axis cs:20.1005025125628,-0.656616457309205)
--(axis cs:10.0502512562814,-0.45455436832764)
--(axis cs:0,-0.277699396817483)
--cycle;

\path [draw=red, fill=red, opacity=0.25]
(axis cs:0,-5.88229124404695)
--(axis cs:0,-6.24805403517312)
--(axis cs:10.0502512562814,-6.98316795094881)
--(axis cs:20.1005025125628,-7.28525514333169)
--(axis cs:30.1507537688442,-7.47492289978182)
--(axis cs:40.2010050251256,-7.62078129779612)
--(axis cs:50.251256281407,-7.71668192353804)
--(axis cs:60.3015075376884,-7.79913720877157)
--(axis cs:70.3517587939699,-7.8672626269254)
--(axis cs:80.4020100502512,-7.9205311279251)
--(axis cs:90.4522613065326,-7.96742318374577)
--(axis cs:100.502512562814,-8.0138450249363)
--(axis cs:110.552763819095,-8.04075570614859)
--(axis cs:120.603015075377,-8.08328895149501)
--(axis cs:130.653266331658,-8.10045173613843)
--(axis cs:140.70351758794,-8.15065656020688)
--(axis cs:150.753768844221,-8.16349160325149)
--(axis cs:160.804020100502,-8.16761790616051)
--(axis cs:170.854271356784,-8.22179168920336)
--(axis cs:180.904522613065,-8.21944940851586)
--(axis cs:190.954773869347,-8.23644066667812)
--(axis cs:190.954773869347,-7.95003961010886)
--(axis cs:190.954773869347,-7.95003961010886)
--(axis cs:180.904522613065,-7.93168504238262)
--(axis cs:170.854271356784,-7.93118322712053)
--(axis cs:160.804020100502,-7.87738130284961)
--(axis cs:150.753768844221,-7.87198604395011)
--(axis cs:140.70351758794,-7.85549810681249)
--(axis cs:130.653266331658,-7.80753566996966)
--(axis cs:120.603015075377,-7.78682732109323)
--(axis cs:110.552763819095,-7.74117164959795)
--(axis cs:100.502512562814,-7.71007963769174)
--(axis cs:90.4522613065326,-7.65865700107438)
--(axis cs:80.4020100502512,-7.60579546588126)
--(axis cs:70.3517587939699,-7.54648990607825)
--(axis cs:60.3015075376884,-7.47178253944074)
--(axis cs:50.251256281407,-7.38225543848004)
--(axis cs:40.2010050251256,-7.27541812536844)
--(axis cs:30.1507537688442,-7.12180689133941)
--(axis cs:20.1005025125628,-6.91711415380228)
--(axis cs:10.0502512562814,-6.60549490340219)
--(axis cs:0,-5.88229124404695)
--cycle;

\addplot [blue, mark=triangle*, mark size=3, mark options={solid,rotate=90}]
table {%
0 1.24589800834656
10.0502510070801 1.18236362934113
20.1005020141602 1.11576080322266
30.1507530212402 1.04572463035583
40.2010040283203 0.972285270690918
50.2512550354004 0.895183205604553
60.3015060424805 0.814651250839233
70.3517608642578 0.730347394943237
80.4020080566406 0.642251014709473
90.452262878418 0.550748705863953
100.502510070801 0.455507278442383
110.552764892578 0.357055187225342
120.603012084961 0.254998922348022
130.653259277344 0.149527192115784
140.703521728516 0.0409756898880005
150.753768920898 -0.0706527233123779
160.804016113281 -0.185504913330078
170.854278564453 -0.303046464920044
180.904525756836 -0.423273086547852
190.954772949219 -0.546412110328674
};
\addlegendentry{\small Prior (N = 1)}
\addplot [red, mark=triangle*, mark size=3, mark options={solid,rotate=90}]
table {%
0 -3.8398118019104
10.0502510070801 -3.97426342964172
20.1005020141602 -4.17198801040649
30.1507530212402 -4.36115026473999
40.2010040283203 -4.53804159164429
50.2512550354004 -4.75966596603394
60.3015060424805 -4.86700534820557
70.3517608642578 -5.11998796463013
80.4020080566406 -5.15160131454468
90.452262878418 -5.34283542633057
100.502510070801 -5.32158041000366
110.552764892578 -5.54748582839966
120.603012084961 -5.593017578125
130.653259277344 -5.69970560073853
140.703521728516 -5.87348699569702
150.753768920898 -6.00191640853882
160.804016113281 -6.05954074859619
170.854278564453 -6.15959930419922
180.904525756836 -6.28391027450562
190.954772949219 -6.47832775115967
};
\addlegendentry{\small Posterior (N = 1)}
\addplot [blue, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
0 -1.37271571159363
20.1005020141602 -1.87403047084808
60.3015060424805 -2.91952085494995
70.3517608642578 -3.17351651191711
80.4020080566406 -3.43225431442261
90.452262878418 -3.68392634391785
100.502510070801 -3.92991065979004
110.552764892578 -4.17323541641235
120.603012084961 -4.40856313705444
130.653259277344 -4.63034915924072
140.703521728516 -4.83384370803833
150.753768920898 -5.04320573806763
160.804016113281 -5.23222827911377
170.854278564453 -5.38818454742432
180.904525756836 -5.52669715881348
190.954772949219 -5.68286514282227
};
\addlegendentry{\small Prior (N = 5)}
\addplot [red, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
0 -5.78368234634399
10.0502510070801 -6.28731441497803
20.1005020141602 -6.7054238319397
30.1507530212402 -7.01446485519409
40.2010040283203 -7.17949914932251
50.2512550354004 -7.32745170593262
60.3015060424805 -7.48990440368652
70.3517608642578 -7.52470254898071
80.4020080566406 -7.63843965530396
90.452262878418 -7.72796297073364
100.502510070801 -7.8355770111084
110.552764892578 -7.85000276565552
120.603012084961 -7.92764377593994
130.653259277344 -8.03104972839355
140.703521728516 -7.94988346099854
150.753768920898 -8.09615993499756
160.804016113281 -8.04897117614746
170.854278564453 -8.15476703643799
180.904525756836 -8.14214324951172
190.954772949219 -8.20853614807129
};
\addlegendentry{\small Posterior (N = 5)}
\addplot [blue, mark=*, mark size=3, mark options={solid}]
table {%
0 -0.306340217590332
10.0502510070801 -0.487745642662048
20.1005020141602 -0.694281101226807
30.1507530212402 -0.901779174804688
40.2010040283203 -1.08853995800018
50.2512550354004 -1.27441251277924
60.3015060424805 -1.43862164020538
70.3517608642578 -1.59907150268555
80.4020080566406 -1.74142932891846
90.452262878418 -1.88248884677887
100.502510070801 -2.01089096069336
110.552764892578 -2.14322304725647
120.603012084961 -2.26374101638794
130.653259277344 -2.37995433807373
140.703521728516 -2.49059343338013
150.753768920898 -2.60335087776184
160.804016113281 -2.71472835540771
170.854278564453 -2.81100726127625
180.904525756836 -2.91172623634338
190.954772949219 -3.00619840621948
};
\addlegendentry{\small Prior (N = 50)}
\addplot [red, mark=*, mark size=3, mark options={solid}]
table {%
0 -6.06517267227173
10.0502510070801 -6.79433155059814
20.1005020141602 -7.1011848449707
30.1507530212402 -7.29836511611938
40.2010040283203 -7.4480996131897
50.2512550354004 -7.54946851730347
60.3015060424805 -7.63545989990234
70.3517608642578 -7.70687627792358
80.4020080566406 -7.7631630897522
90.452262878418 -7.81304025650024
100.502510070801 -7.86196231842041
110.552764892578 -7.89096355438232
120.603012084961 -7.93505811691284
130.653259277344 -7.95399379730225
140.703521728516 -8.00307750701904
150.753768920898 -8.01773929595947
160.804016113281 -8.02250003814697
170.854278564453 -8.07648754119873
180.904525756836 -8.0755672454834
190.954772949219 -8.09323978424072
};
\addlegendentry{\small Posterior (N = 50)}
\end{axis}

\end{tikzpicture}


==> sections/rl_bench_rerun.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
         \centering
	\tiny
\begin{tabular}{@{}llll@{}}
\toprule
                           & \textbf{Reach Target}        & \textbf{Close Box}                    & \textbf{Water Plants}        \\ \midrule
                           &                              & \textbf{Low Dimensional Conditioning} &                              \\ \midrule
\textbf{ProMP}             & 0.00769 +/- 0.00004          & \textbf{0.16404 +/- 0.03307}          & \textbf{0.36887 +/- 0.04911} \\
\textbf{CNMP}              & 0.17298   +/- 0.02478        & 0.39629 +/-        0.13847            & 0.7147+/-0.36565             \\
\textbf{VAE-CNMP}          & 0.33666  +/- 0.23263         & 0.41986 +/- 0.12136                   & 0.57952+/-0.16628            \\
\textbf{DeepProMP}         & 0.00171 +/- 0.00026          & 0.18718 +/- 0.01217                   & 0.41231+/- 0.02825           \\
\textbf{Marginal DeeProMP} & \textbf{0.0002 +/- 0.00009}  & 0.18113 +/- 0.00758                   & 0.42016+/-0.04269            \\ \midrule
                           &                              & \textbf{Image Conditioning}           &                              \\ \midrule
\textbf{ProMP}             & NA                           & NA                                    & NA                           \\
\textbf{CNMP}              & \textbf{0.00062 +/- 0.00002} & 0.36341 +/- 0.04499                   & 0.74135+/-0.04855            \\
\textbf{Vae-CNMP}          & 0.0008 +/-       0.00008     & 0.31899 +/- 0.04261                   & 0.78985+/-0.06483            \\
\textbf{DeePromp}          & 0.00139 +/- 0.00045          & 0.18284 +/- 0.01162                   & 0.50485+/-0.02173            \\
\textbf{Marginal DeeProMP} & 0.00286 +/- 0.00181          & \textbf{0.15913 +/- 0.00802}          & \textbf{0.41646+/-0.02055}   \\ \midrule
                           &                              & \textbf{Both}                         &                              \\ \midrule
ProMP                      & NA                           & NA                                    & NA                           \\
\textbf{CNMP}              & 0.00059 +/- 0.00003          & 0.20315 +/- 0.01118                   & 0.52052+/-0.11496            \\
\textbf{Vae-CNMP}          & \textbf{0.00076 +/- 0.00009} & 0.1896 +/- 0.03534                    & 0.41769+/-0.05017            \\
\textbf{DeePromp}          & 0.00094 +/- 0.00026          & 0.18302 +/- 0.01183                   & 0.48454+/-0.02201            \\
\textbf{Marginal DeeProMP} & 0.00109 +/- 0.0011           & \textbf{0.16357+/- 0.00359}           & \textbf{0.40394+/-0.01481}   \\ \midrule
                           &                              & \textbf{Via Point Reconstruction}     &                              \\ \midrule
\textbf{ProMP}             & \textbf{0.00004 +/- 0.00001} & \textbf{0.0012 +/- 0.00019}           & \textbf{0.00158 +/- 0.00037} \\
\textbf{CNMP}              & 0.16545 +/- 0.0209           & 0.54709+/- 0.07269                    & 0.86325+/-0.46799            \\
\textbf{Vae-CNMP}          & 0.33692 +/- 0.23559          & 0.54116+/- 0.1322                     & 0.5399+/-0.07288             \\
\textbf{DeePromp}          & 0.00012 +/- 0.00002          & 0.02172+/- 0.00104                    & 0.02535+/-0.00288            \\
\textbf{Marginal DeeProMP} & 0.00008  +/-       0.00004   & 0.02566+/- 0.00172                    & 0.0352+/- 0.00578            \\ \midrule
                           &                              & \textbf{Aggregate}                    &                              \\ \midrule
\textbf{ProMP}             & NA                           & NA                                    & NA                           \\
\textbf{CNMP}              & 0.08491 +/- 0.01136          & 0.37748+/-0.04752                     & 0.68425+/-0.20441            \\
\textbf{Vae-CNMP}          & 0.16879  +/-        0.11704  & 0.3674+/- 0.06763                     & 0.60745+/-0.09211            \\
\textbf{DeePromp}          & \textbf{0.00104 +/- 0.00024} & 0.14369+/-0.00802                     & 0.35676+/-0.01416            \\
\textbf{Marginal DeeProMP} & 0.00106 +/- 0.00073          & \textbf{0.13237 +/- 0.00365}          & \textbf{0.31894+/- 0.01776}  \\ \bottomrule
\end{tabular}
\caption{DeepProMPs and CNMPs compared on RLBench~\cite{james_rlbench_2020} tasks. DeepProMPs (ours) exhibit lower reconstruction error, higher precision in via-point conditioning. Apparently, the higher accuracy does not have a direct effect on the task performance, as VAE-CNMPs and DeepProMPs have similar success rate.  Intervals denote the standard deviation, ProMP results are boostrapped over 4000 subsets of results to produce confidence intervals \label{tab:rlbench}\label{tab:rreal-robot}}
\end{table}

==> sections/rlbench_results.tex <==
\begin{table}[]
	\centering
	\tiny
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{1}{l}{}  & \texttt{Reach Target}        & \texttt{Close Box}  & \texttt{Water Plants}  & \texttt{Clean Table} \\
\midrule 
 & \multicolumn{3}{c}{Task Reconstruction}   \\                   %    & \multicolumn{3}{c}{Way Point Reconstruction}                                & \multicolumn{3}{c}{Success Rate}                            \\ 
  \midrule
\textbf{ProMP}        &  0.02285 +/- 0.00173 & 0.1737 +/- 0.0328    & 0.2871 +/- 0.04212   & 0.08212 +/- 0.0283	  \\
\textbf{CNMP}         & 5.35e-03 +/- 6.96e-04 & 0.2124 +/- 0.01294  & 0.3122 +/- 0.01177   & 0.08176 +/- 0.00825\\
\textbf{VAE-CNMP} & \textbf{5.21e-05 +/- 8.25e-06} & 0.1676 +/- 0.008287 & \textbf{0.2482 +/- 0.04568} & 0.0222 +/- 0.01185   \\
\textbf{DeepProMPs}          & \textbf{4.56e-05 +/- 4.82e-06} & \textbf{0.1461 +/- 0.012}     & \textbf{0.2719 +/- 0.02877}  & 0.0225 +/- 0.0065    \\
 \midrule \multicolumn{1}{l}{}  & \multicolumn{3}{c}{Via-Point Reconstruction}  & -  \\       
 \midrule
\textbf{ProMP}        & 0.0007 +/- 0.00014	 & 0.00235 +/- 0.00016     & 0.01357 +/- 0.00293  & 0.02826 +/- 0.00065	  \\
\textbf{CNMP}        & 3.63e-01 +/- 4.51e-02 & 0.654 +/- 0.05761      & 0.7873    +/-    0.09878    & 0.0439 +/- 0.003546	  \\
\textbf{VAE-CNMP} & 6.06e-05 +/- 1.66e-05 & 0.003686 +/- 0.0004681 & \textbf{0.001774    +/-  0.0003767 }  & 0.02218 +/- 0.02252 \\
\textbf{DeepProMPs}           & \textbf{4.33e-05 +/- 5.49e-06} & \textbf{0.001937 +/- 0.0004681} & \textbf{0.001684  +/-   0.0005754} &  0.01112 +/- 0.00363  \\
\midrule \multicolumn{1}{l}{}  & \multicolumn{3}{c}{Success Rate}   \\      
\midrule 
\textbf{ProMP}         & 0.698 +/- 0.117 & 0.1504 +/- 0.092    & 0.05198 +/- 0.05638     & -  \\
\textbf{CNMP}         & 0.78 +/- 0.07141 & 0.19 +/- 0.0995    & 0.005 +/- 0.015     & 0.0  \\
\textbf{VAE-CNMP} &\textbf{1.0}                & \textbf{0.505 +/- 0.1823}   & \textbf{0.2625 +/- 0.09922}  &  0.8553 +/- 0.09919  \\
\textbf{DeepProMPs}          & \textbf{1.0}                & \textbf{0.495 +/- 0.065}    & \textbf{0.255 +/- 0.1474}    & 0.84167 +/- 0.1493   \\ \bottomrule
 \bottomrule
\end{tabular}
\vspace{1em}
\caption{DeepProMPs and CNMPs compared on RLBench~\cite{james_rlbench_2020} tasks. DeepProMPs (ours) exhibit lower reconstruction error, higher precision in via-point conditioning. Apparently, the higher accuracy does not have a direct effect on the task performance, as VAE-CNMPs and DeepProMPs have similar success rate.  Intervals denote the standard deviation, ProMP results are boostrapped over 4000 subsets of results to produce confidence intervals \label{tab:rlbench}\label{tab:rreal-robot}}
\end{table}

